Efficient Image Dataset Classification Difficulty Estimation for Predicting Deep-Learning Accuracy

In the deep-learning community new algorithms are published at an incredible pace. Therefore, solving an image classification problem for new datasets becomes a challenging task, as it requires to re-evaluate published algorithms and their different configurations in order to find a close to optimal classifier. To facilitate this process, before biasing our decision towards a class of neural networks or running an expensive search over the network space, we propose to estimate the classification difficulty of the dataset. Our method computes a single number that characterizes the dataset difficulty 27x faster than training state-of-the-art networks. The proposed method can be used in combination with network topology and hyper-parameter search optimizers to efficiently drive the search towards promising neural-network configurations.

==> preamble/custom.tex <==
% ---------------------------------------------------------------------
% ADDED by Florian, allows ä,ü etc.
% Determines the input encoding.
\usepackage[%
 utf8,
% latin1
]{inputenc}

% ---------------------------------------------------------------------
% Determines the output encoding.
\usepackage[T1]{fontenc}
% ---------------------------------------------------------------------

% *** MISC UTILITY PACKAGES ***

\usepackage{color}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{placeins}
\usepackage[para]{threeparttable}
\usepackage{multirow}
\usepackage{multicol}

% some useful commands for text coloring
\usepackage{color}
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\definecolor{darkblue}{rgb}{0.0, 0.0, 0.55}
\definecolor{lightblue}{rgb}{0.0, 0.4, 0.8}
\definecolor{darkgreen}{rgb}{0.00, 0.44, 0.0}
\definecolor{forestgreen}{rgb}{0.0, 0.27, 0.13}
\definecolor{internationalorange}{rgb}{1.0, 0.31, 0.0}
\newcommand{\todo}[1]{{\color{red}{\bf [{\sl #1}]}}}

% MARK DELTA
\newcommand{\rev}[1]{{\color{green}#1}}
\newcommand{\del}[1]{{\color{red}#1}}

% FINAL
% \newcommand{\rev}[1]{#1} % copy through
% \newcommand{\del}[1]{}   % delete

% for tables
% ------------------------------------------------------------------------------

\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\newcolumntype{x}[1]{>{\centering\arraybackslash\hspace{0pt}}p{#1}}
